Formation of Thermal Vortex Rings

An evolution of a spherical region, subjected to uniform buoyancy force, is investigated. Incompressibility and axial symmetry are assumed, together with a buoyancy discontinuity at the boundary. The boundary turns into a vortex sheet and the system evolves into a ring. Contrary to the case of mechanically generated rings, buoyancy-driven rings are unstable. This is due to the generation of negative vorticity at the bottom. Furthermore, a sequence of Kelvin-Helmholtz instabilities arises along the buoyancy anomaly boundary. This sequence transfers the energy toward large scales with $\kappa^{-3}$ distribution. The vortex blob method has been used to simulate the system numerically. An optimization algorithm, used previously in two dimensions, has been extended to the axisymmetric case. It reduces computational complexity from $N^2$ to $N \log N$, where N is the number of nodes. Additionally, a new algorithm has been developed as a remedy for the exponential growth of the number of nodes required. It exploits a tendency of the vortex sheet to form many parallel stripes, by merging them together.

==> fig_statement.tex <==
\begin{tikzpicture}[scale=2]
\draw[black,fill=myBlue] (0,0) circle(1);
%\draw (0,0) ellipse (1 and .2);
\draw plot[domain=pi:2*pi] ({cos(\x r)},{0.3*sin(\x r)});
\draw[dashed] plot[domain=0:pi] ({cos(\x r)},{0.3*sin(\x r)});

% Axes
\draw[->] (0,0)--({0.2588*1.4},{-0.9659*0.3*1.4}) node[right] {$x$};
\draw[->] (0,0)--(1.2,0) node[above] {$r$};
\draw[->] (0,0)--(0,1.2) node[above] {$z$};

\end{tikzpicture}



==> figures/fig_dynnikova_coords.tex <==
\draw[gray, thin, opacity=\opp](29.267520 cm, 1.824420 cm)
--(29.265000 cm, 1.860870 cm)
--(29.262510 cm, 1.897290 cm)
--(29.261880 cm, 1.933200 cm)
--(29.261250 cm, 1.969110 cm)
--(29.262720 cm, 2.003520 cm)
--(29.264220 cm, 2.037930 cm)
--(29.267100 cm, 2.071530 cm)
--(29.269980 cm, 2.105130 cm)
--(29.274390 cm, 2.135850 cm)
--(29.278830 cm, 2.166540 cm)
--(29.284500 cm, 2.196270 cm)
--(29.290200 cm, 2.226030 cm)
--(29.304780 cm, 2.280510 cm)
--(29.322240 cm, 2.332440 cm)
--(29.336880 cm, 2.362260 cm)
--(29.351550 cm, 2.392080 cm)
--(29.368590 cm, 2.418810 cm)
--(29.385630 cm, 2.445510 cm)
--(29.424000 cm, 2.485950 cm)
--(29.464710 cm, 2.519520 cm)
--(29.501880 cm, 2.537430 cm)
--(29.538510 cm, 2.551320 cm)
--(29.573280 cm, 2.557950 cm)
--(29.606580 cm, 2.562810 cm)
--(29.654070 cm, 2.559570 cm)
--(29.696400 cm, 2.554380 cm)
--(29.730390 cm, 2.546970 cm)
--(29.761950 cm, 2.542050 cm)
--(29.800620 cm, 2.529840 cm)
--(29.834310 cm, 2.521980 cm)
--(29.858910 cm, 2.512740 cm)
--(29.882520 cm, 2.506710 cm)
--(29.903490 cm, 2.490210 cm)
--(29.919390 cm, 2.474190 cm)
--(29.923710 cm, 2.454270 cm)
--(29.924910 cm, 2.436270 cm)
--(29.907840 cm, 2.413230 cm)
--(29.886360 cm, 2.394480 cm)
--(29.847630 cm, 2.378730 cm)
--(29.805030 cm, 2.366040 cm)
--(29.775750 cm, 2.363670 cm)
--(29.746470 cm, 2.361300 cm)
--(29.690400 cm, 2.362770 cm)
--(29.662020 cm, 2.369040 cm)
--(29.634630 cm, 2.375790 cm)
--(29.616780 cm, 2.386350 cm)
--(29.607540 cm, 2.399040 cm)
--(29.609190 cm, 2.410020 cm)
--(29.617710 cm, 2.418300 cm)
--(29.627430 cm, 2.427240 cm)
--(29.634780 cm, 2.436990 cm)
--(29.638440 cm, 2.447010 cm)
--(29.633070 cm, 2.460180 cm)
--(29.609190 cm, 2.476380 cm)
--(29.579070 cm, 2.481570 cm)
--(29.548290 cm, 2.484420 cm)
--(29.503380 cm, 2.472600 cm)
--(29.457930 cm, 2.448180 cm)
--(29.431170 cm, 2.423310 cm)
--(29.406360 cm, 2.394990 cm)
--(29.383800 cm, 2.360400 cm)
--(29.363370 cm, 2.322990 cm)
--(29.347800 cm, 2.280480 cm)
--(29.334300 cm, 2.236050 cm)
--(29.323440 cm, 2.188050 cm)
--(29.314650 cm, 2.138760 cm)
--(29.310030 cm, 2.086680 cm)
--(29.307150 cm, 2.033520 cm)
--(29.309220 cm, 1.999080 cm)
--(29.311290 cm, 1.964640 cm)
--(29.318910 cm, 1.960500 cm)
--(29.328120 cm, 1.966230 cm)
--(29.335980 cm, 1.995000 cm)
--(29.344620 cm, 2.020410 cm)
--(29.358300 cm, 2.066850 cm)
--(29.374710 cm, 2.108460 cm)
--(29.388090 cm, 2.138910 cm)
--(29.401500 cm, 2.169360 cm)
--(29.418900 cm, 2.198250 cm)
--(29.437620 cm, 2.222370 cm)
--(29.465760 cm, 2.251590 cm)
--(29.496930 cm, 2.271630 cm)
--(29.538480 cm, 2.287950 cm)
--(29.587380 cm, 2.295180 cm)
--(29.623890 cm, 2.298390 cm)
--(29.662950 cm, 2.299470 cm)
--(29.708010 cm, 2.300970 cm)
--(29.755080 cm, 2.302620 cm)
--(29.805420 cm, 2.305680 cm)
--(29.853930 cm, 2.309220 cm)
--(29.897160 cm, 2.313060 cm)
--(29.937300 cm, 2.318550 cm)
--(29.967900 cm, 2.323710 cm)
--(29.996820 cm, 2.330790 cm)
--(30.020940 cm, 2.338770 cm)
--(30.043830 cm, 2.348790 cm)
--(30.077250 cm, 2.366100 cm)
--(30.105660 cm, 2.388450 cm)
--(30.129660 cm, 2.409870 cm)
--(30.148890 cm, 2.430930 cm)
--(30.163290 cm, 2.445270 cm)
--(30.176670 cm, 2.462640 cm)
--(30.195930 cm, 2.483610 cm)
--(30.210750 cm, 2.500320 cm)
--(30.222360 cm, 2.509980 cm)
--(30.232200 cm, 2.519100 cm)
--(30.240390 cm, 2.520900 cm)
--(30.247650 cm, 2.522910 cm)
--(30.254700 cm, 2.516490 cm)
--(30.261150 cm, 2.512980 cm)
--(30.266460 cm, 2.502540 cm)
--(30.271440 cm, 2.496870 cm)
--(30.277770 cm, 2.466030 cm)
--(30.281130 cm, 2.431800 cm)
--(30.278130 cm, 2.383290 cm)
--(30.271590 cm, 2.336730 cm)
--(30.263040 cm, 2.305710 cm)
--(30.254490 cm, 2.274660 cm)
--(30.243780 cm, 2.247390 cm)
--(30.233040 cm, 2.220120 cm)
--(30.213240 cm, 2.186490 cm)
--(30.193440 cm, 2.152890 cm)
--(30.171810 cm, 2.127120 cm)
--(30.150180 cm, 2.101350 cm)
--(30.120660 cm, 2.078820 cm)
--(30.091140 cm, 2.056290 cm)
--(30.061200 cm, 2.041590 cm)
--(30.031260 cm, 2.026860 cm)
--(29.979720 cm, 2.015250 cm)
--(29.932290 cm, 2.011290 cm)
--(29.890770 cm, 2.016780 cm)
--(29.853780 cm, 2.025150 cm)
--(29.823540 cm, 2.040450 cm)
--(29.795970 cm, 2.055810 cm)
--(29.779440 cm, 2.073750 cm)
--(29.763900 cm, 2.090460 cm)
--(29.755320 cm, 2.121870 cm)
--(29.761410 cm, 2.148660 cm)
--(29.783820 cm, 2.167290 cm)
--(29.810430 cm, 2.182110 cm)
--(29.839140 cm, 2.185440 cm)
--(29.867880 cm, 2.188770 cm)
--(29.905170 cm, 2.183100 cm)
--(29.925060 cm, 2.172780 cm)
--(29.931360 cm, 2.161950 cm)
--(29.932050 cm, 2.151660 cm)
--(29.933640 cm, 2.140830 cm)
--(29.940690 cm, 2.130030 cm)
--(29.957250 cm, 2.121960 cm)
--(29.991120 cm, 2.121450 cm)
--(30.042840 cm, 2.144820 cm)
--(30.066480 cm, 2.171610 cm)
--(30.084630 cm, 2.201970 cm)
--(30.083610 cm, 2.222220 cm)
--(30.079350 cm, 2.241990 cm)
--(30.056730 cm, 2.254020 cm)
--(30.023430 cm, 2.264130 cm)
--(29.993910 cm, 2.265420 cm)
--(29.960190 cm, 2.267940 cm)
--(29.914110 cm, 2.268780 cm)
--(29.859120 cm, 2.269260 cm)
--(29.801910 cm, 2.266620 cm)
--(29.771430 cm, 2.264040 cm)
--(29.740920 cm, 2.261460 cm)
--(29.687430 cm, 2.253030 cm)
--(29.638020 cm, 2.241750 cm)
--(29.607180 cm, 2.226960 cm)
--(29.579280 cm, 2.208840 cm)
--(29.562210 cm, 2.189460 cm)
--(29.546550 cm, 2.164950 cm)
--(29.541900 cm, 2.144520 cm)
--(29.538450 cm, 2.120190 cm)
--(29.541960 cm, 2.097660 cm)
--(29.548590 cm, 2.073360 cm)
--(29.556810 cm, 2.063970 cm)
--(29.564730 cm, 2.050920 cm)
--(29.576040 cm, 2.039880 cm)
--(29.588340 cm, 2.026350 cm)
--(29.605950 cm, 2.015250 cm)
--(29.626200 cm, 2.002170 cm)
--(29.652750 cm, 1.989690 cm)
--(29.685420 cm, 1.975470 cm)
--(29.707140 cm, 1.969860 cm)
--(29.730150 cm, 1.961580 cm)
--(29.757990 cm, 1.955190 cm)
--(29.789730 cm, 1.948110 cm)
--(29.829150 cm, 1.943460 cm)
--(29.875440 cm, 1.940760 cm)
--(29.902740 cm, 1.942470 cm)
--(29.931390 cm, 1.944270 cm)
--(29.963250 cm, 1.949910 cm)
--(29.996850 cm, 1.956540 cm)
--(30.035820 cm, 1.970970 cm)
--(30.076470 cm, 1.988190 cm)
--(30.118500 cm, 2.014710 cm)
--(30.160620 cm, 2.046030 cm)
--(30.181560 cm, 2.067450 cm)
--(30.202500 cm, 2.088870 cm)
--(30.221820 cm, 2.114010 cm)
--(30.241140 cm, 2.139180 cm)
--(30.258060 cm, 2.168670 cm)
--(30.274950 cm, 2.198160 cm)
--(30.288810 cm, 2.230650 cm)
--(30.302670 cm, 2.263140 cm)
--(30.313590 cm, 2.300550 cm)
--(30.324480 cm, 2.337990 cm)
--(30.331740 cm, 2.377470 cm)
--(30.338970 cm, 2.416920 cm)
--(30.341700 cm, 2.458950 cm)
--(30.344430 cm, 2.500980 cm)
--(30.342330 cm, 2.544030 cm)
--(30.340260 cm, 2.587080 cm)
--(30.333510 cm, 2.632140 cm)
--(30.324750 cm, 2.677080 cm)
--(30.313050 cm, 2.721720 cm)
--(30.299580 cm, 2.765940 cm)
--(30.283260 cm, 2.810130 cm)
--(30.265260 cm, 2.853810 cm)
--(30.245670 cm, 2.896800 cm)
--(30.224760 cm, 2.939340 cm)
--(30.201480 cm, 2.982540 cm)
--(30.177330 cm, 3.025380 cm)
--(30.151980 cm, 3.067770 cm)
--(30.125880 cm, 3.109890 cm)
--(30.098730 cm, 3.151890 cm)
--(30.071070 cm, 3.193770 cm)
--(30.042810 cm, 3.235680 cm)
--(30.014220 cm, 3.277650 cm)
--(29.985210 cm, 3.320040 cm)
--(29.956110 cm, 3.362790 cm)
--(29.927310 cm, 3.405960 cm)
--(29.898810 cm, 3.449640 cm)
--(29.871300 cm, 3.493830 cm)
--(29.844600 cm, 3.538560 cm)
--(29.819340 cm, 3.583680 cm)
--(29.795130 cm, 3.629280 cm)
--(29.772990 cm, 3.674280 cm)
--(29.751810 cm, 3.719490 cm)
--(29.732040 cm, 3.764550 cm)
--(29.713230 cm, 3.809940 cm)
--(29.696070 cm, 3.854610 cm)
--(29.680020 cm, 3.899670 cm)
--(29.665590 cm, 3.944760 cm)
--(29.652330 cm, 3.990120 cm)
--(29.642430 cm, 4.034190 cm)
--(29.632560 cm, 4.078260 cm)
--(29.626560 cm, 4.121790 cm)
--(29.620530 cm, 4.165290 cm)
--(29.618760 cm, 4.206720 cm)
--(29.617020 cm, 4.248150 cm)
--(29.618940 cm, 4.287330 cm)
--(29.620890 cm, 4.326540 cm)
--(29.626200 cm, 4.361250 cm)
--(29.631540 cm, 4.395990 cm)
--(29.639250 cm, 4.427400 cm)
--(29.646960 cm, 4.458780 cm)
--(29.656740 cm, 4.486290 cm)
--(29.666550 cm, 4.513830 cm)
--(29.688420 cm, 4.562310 cm)
--(29.711310 cm, 4.601730 cm)
--(29.734380 cm, 4.635870 cm)
--(29.756910 cm, 4.664040 cm)
--(29.778360 cm, 4.688460 cm)
--(29.798190 cm, 4.706040 cm)
--(29.816070 cm, 4.723560 cm)
--(29.832540 cm, 4.736340 cm)
--(29.847780 cm, 4.749360 cm)
--(29.873370 cm, 4.768380 cm)
--(29.893170 cm, 4.785960 cm)
--(29.907690 cm, 4.800000 cm)
--(29.918640 cm, 4.815210 cm)
--(29.927160 cm, 4.829790 cm)
--(29.932800 cm, 4.848480 cm)
--(29.937510 cm, 4.864440 cm)
--(29.940690 cm, 4.882980 cm)
--(29.943900 cm, 4.920930 cm)
--(29.945760 cm, 4.956000 cm)
--(29.946060 cm, 4.991850 cm)
--(29.947530 cm, 5.022750 cm)
--(29.947920 cm, 5.054160 cm)
--(29.952600 cm, 5.077890 cm)
--(29.956710 cm, 5.100240 cm)
--(29.964090 cm, 5.107500 cm)
--(29.970630 cm, 5.114160 cm)
--(29.982750 cm, 5.094660 cm)
--(29.994750 cm, 5.072160 cm)
--(30.012750 cm, 5.025270 cm)
--(30.031500 cm, 4.975380 cm)
--(30.042480 cm, 4.942140 cm)
--(30.053460 cm, 4.908900 cm)
--(30.064830 cm, 4.875030 cm)
--(30.076170 cm, 4.841190 cm)
--(30.087840 cm, 4.804260 cm)
--(30.099510 cm, 4.767360 cm)
--(30.110370 cm, 4.729950 cm)
--(30.121230 cm, 4.692570 cm)
--(30.131460 cm, 4.644390 cm)
--(30.141720 cm, 4.596210 cm)
--(30.147780 cm, 4.549440 cm)
--(30.153870 cm, 4.502700 cm)
--(30.153930 cm, 4.459410 cm)
--(30.153990 cm, 4.416150 cm)
--(30.149910 cm, 4.377090 cm)
--(30.145830 cm, 4.338060 cm)
--(30.133110 cm, 4.293240 cm)
--(30.118110 cm, 4.252860 cm)
--(30.100050 cm, 4.220790 cm)
--(30.081270 cm, 4.192380 cm)
--(30.041130 cm, 4.160310 cm)
--(30.001020 cm, 4.146300 cm)
--(29.967450 cm, 4.155060 cm)
--(29.937300 cm, 4.173090 cm)
--(29.909670 cm, 4.217070 cm)
--(29.907060 cm, 4.234920 cm)
--(29.907000 cm, 4.255140 cm)
--(29.910930 cm, 4.272240 cm)
--(29.917440 cm, 4.277760 cm)
--(29.925090 cm, 4.283280 cm)
--(29.931750 cm, 4.288650 cm)
--(29.939940 cm, 4.306410 cm)
--(29.947050 cm, 4.323570 cm)
--(29.955210 cm, 4.353540 cm)
--(29.959980 cm, 4.383000 cm)
--(29.960640 cm, 4.419840 cm)
--(29.958270 cm, 4.447890 cm)
--(29.955150 cm, 4.467720 cm)
--(29.949990 cm, 4.486680 cm)
--(29.941050 cm, 4.506540 cm)
--(29.911830 cm, 4.536990 cm)
--(29.887860 cm, 4.545180 cm)
--(29.862870 cm, 4.551630 cm)
--(29.817450 cm, 4.536270 cm)
--(29.794830 cm, 4.520160 cm)
--(29.772030 cm, 4.501410 cm)
--(29.753490 cm, 4.474500 cm)
--(29.735460 cm, 4.444920 cm)
--(29.720100 cm, 4.409730 cm)
--(29.706300 cm, 4.371510 cm)
--(29.697330 cm, 4.328340 cm)
--(29.690760 cm, 4.282770 cm)
--(29.688240 cm, 4.234200 cm)
--(29.688750 cm, 4.184190 cm)
--(29.695560 cm, 4.127430 cm)
--(29.700810 cm, 4.098780 cm)
--(29.706090 cm, 4.070130 cm)
--(29.713530 cm, 4.041420 cm)
--(29.720970 cm, 4.012710 cm)
--(29.729910 cm, 3.984360 cm)
--(29.738820 cm, 3.955980 cm)
--(29.756700 cm, 3.912510 cm)
--(29.774580 cm, 3.869040 cm)
--(29.793990 cm, 3.828540 cm)
--(29.813430 cm, 3.788040 cm)
--(29.828550 cm, 3.762840 cm)
--(29.843700 cm, 3.737670 cm)
--(29.859570 cm, 3.713640 cm)
--(29.875440 cm, 3.689610 cm)
--(29.895840 cm, 3.669660 cm)
--(29.916810 cm, 3.651690 cm)
--(29.923740 cm, 3.656700 cm)
--(29.931000 cm, 3.662760 cm)
--(29.933940 cm, 3.678210 cm)
--(29.936820 cm, 3.695190 cm)
--(29.935170 cm, 3.724320 cm)
--(29.934210 cm, 3.754830 cm)
--(29.932050 cm, 3.791430 cm)
--(29.932680 cm, 3.827760 cm)
--(29.933640 cm, 3.855720 cm)
--(29.939940 cm, 3.878160 cm)
--(29.949300 cm, 3.902940 cm)
--(29.956860 cm, 3.913800 cm)
--(29.966730 cm, 3.922650 cm)
--(29.978160 cm, 3.935580 cm)
--(29.993430 cm, 3.945870 cm)
--(30.011070 cm, 3.959850 cm)
--(30.032640 cm, 3.973770 cm)
--(30.057450 cm, 3.997170 cm)
--(30.086190 cm, 4.026060 cm)
--(30.101040 cm, 4.047510 cm)
--(30.117210 cm, 4.069680 cm)
--(30.133050 cm, 4.097640 cm)
--(30.149970 cm, 4.127670 cm)
--(30.166410 cm, 4.171590 cm)
--(30.182880 cm, 4.220070 cm)
--(30.189030 cm, 4.249710 cm)
--(30.195180 cm, 4.279320 cm)
--(30.199770 cm, 4.312110 cm)
--(30.204390 cm, 4.344870 cm)
--(30.205230 cm, 4.385040 cm)
--(30.206070 cm, 4.425210 cm)
--(30.203520 cm, 4.468920 cm)
--(30.200970 cm, 4.512630 cm)
--(30.193590 cm, 4.560750 cm)
--(30.186210 cm, 4.608840 cm)
--(30.175230 cm, 4.658730 cm)
--(30.164280 cm, 4.708620 cm)
--(30.149880 cm, 4.761480 cm)
--(30.135480 cm, 4.814370 cm)
--(30.120510 cm, 4.867050 cm)
--(30.105510 cm, 4.919730 cm)
--(30.091380 cm, 4.972530 cm)
--(30.077220 cm, 5.025360 cm)
--(30.065010 cm, 5.077170 cm)
--(30.052770 cm, 5.128980 cm)
--(30.043410 cm, 5.178420 cm)
--(30.034050 cm, 5.227860 cm)
--(30.027090 cm, 5.275260 cm)
--(30.020130 cm, 5.322630 cm)
--(30.017430 cm, 5.366370 cm)
--(30.014760 cm, 5.410080 cm)
--(30.015510 cm, 5.451180 cm)
--(30.016290 cm, 5.492250 cm)
--(30.021390 cm, 5.523690 cm)
--(30.026490 cm, 5.555100 cm)
--(30.033600 cm, 5.584410 cm)
--(30.040710 cm, 5.613690 cm)
--(30.060630 cm, 5.664090 cm)
--(30.082710 cm, 5.710350 cm)
--(30.107790 cm, 5.744490 cm)
--(30.133890 cm, 5.775090 cm)
--(30.162180 cm, 5.798040 cm)
--(30.190560 cm, 5.817900 cm)
--(30.241200 cm, 5.833290 cm)
--(30.290550 cm, 5.836080 cm)
--(30.334260 cm, 5.825850 cm)
--(30.373980 cm, 5.810130 cm)
--(30.398580 cm, 5.792400 cm)
--(30.423180 cm, 5.774700 cm)
--(30.462210 cm, 5.739030 cm)
--(30.490200 cm, 5.706990 cm)
--(30.515010 cm, 5.679090 cm)
--(30.543990 cm, 5.637210 cm)
--(30.567810 cm, 5.603220 cm)
--(30.578490 cm, 5.577600 cm)
--(30.588540 cm, 5.555100 cm)
--(30.590520 cm, 5.536260 cm)
--(30.592920 cm, 5.518770 cm)
--(30.581370 cm, 5.497440 cm)
--(30.565710 cm, 5.483400 cm)
--(30.537900 cm, 5.488470 cm)
--(30.509250 cm, 5.496660 cm)
--(30.483240 cm, 5.514150 cm)
--(30.457170 cm, 5.532960 cm)
--(30.432690 cm, 5.555790 cm)
--(30.408180 cm, 5.578650 cm)
--(30.387600 cm, 5.604780 cm)
--(30.367830 cm, 5.630130 cm)
--(30.355320 cm, 5.656110 cm)
--(30.356430 cm, 5.668020 cm)
--(30.364380 cm, 5.673420 cm)
--(30.375960 cm, 5.674230 cm)
--(30.386520 cm, 5.676930 cm)
--(30.393180 cm, 5.683170 cm)
--(30.391260 cm, 5.700120 cm)
--(30.368460 cm, 5.734320 cm)
--(30.337680 cm, 5.757510 cm)
--(30.304020 cm, 5.775510 cm)
--(30.274530 cm, 5.778900 cm)
--(30.244560 cm, 5.779590 cm)
--(30.212670 cm, 5.769870 cm)
--(30.180960 cm, 5.756400 cm)
--(30.147660 cm, 5.724780 cm)
--(30.115740 cm, 5.687640 cm)
--(30.094320 cm, 5.645040 cm)
--(30.075000 cm, 5.598330 cm)
--(30.066690 cm, 5.557260 cm)
--(30.062700 cm, 5.520210 cm)
--(30.070140 cm, 5.517480 cm)
--(30.083790 cm, 5.530800 cm)
--(30.101640 cm, 5.559480 cm)
--(30.122610 cm, 5.582280 cm)
--(30.158160 cm, 5.611410 cm)
--(30.181200 cm, 5.622420 cm)
--(30.204720 cm, 5.627070 cm)
--(30.242430 cm, 5.626170 cm)
--(30.281970 cm, 5.610060 cm)
--(30.306990 cm, 5.594700 cm)
--(30.332280 cm, 5.574990 cm)
--(30.361050 cm, 5.550510 cm)
--(30.391470 cm, 5.523030 cm)
--(30.427560 cm, 5.490900 cm)
--(30.464190 cm, 5.458290 cm)
--(30.499230 cm, 5.427510 cm)
--(30.531780 cm, 5.399790 cm)
--(30.558780 cm, 5.378340 cm)
--(30.584640 cm, 5.361840 cm)
--(30.607290 cm, 5.350800 cm)
--(30.630030 cm, 5.345070 cm)
--(30.662520 cm, 5.343240 cm)
--(30.692550 cm, 5.351640 cm)
--(30.715470 cm, 5.363190 cm)
--(30.737310 cm, 5.381490 cm)
--(30.765270 cm, 5.410140 cm)
--(30.787080 cm, 5.443620 cm)
--(30.798480 cm, 5.458140 cm)
--(30.808740 cm, 5.475810 cm)
--(30.815070 cm, 5.478840 cm)
--(30.821490 cm, 5.487090 cm)
--(30.825120 cm, 5.465580 cm)
--(30.825420 cm, 5.434710 cm)
--(30.815610 cm, 5.380890 cm)
--(30.800220 cm, 5.328660 cm)
--(30.786480 cm, 5.300550 cm)
--(30.772770 cm, 5.272410 cm)
--(30.756540 cm, 5.248170 cm)
--(30.740340 cm, 5.223900 cm)
--(30.719130 cm, 5.203860 cm)
--(30.697920 cm, 5.183850 cm)
--(30.652410 cm, 5.155650 cm)
--(30.607410 cm, 5.144670 cm)
--(30.563550 cm, 5.144880 cm)
--(30.530520 cm, 5.157840 cm)
--(30.499440 cm, 5.173710 cm)
--(30.476280 cm, 5.199690 cm)
--(30.456360 cm, 5.227410 cm)
--(30.448710 cm, 5.256990 cm)
--(30.454350 cm, 5.268810 cm)
--(30.465720 cm, 5.271180 cm)
--(30.481020 cm, 5.268360 cm)
--(30.496650 cm, 5.261070 cm)
--(30.511140 cm, 5.256570 cm)
--(30.525150 cm, 5.259630 cm)
--(30.532770 cm, 5.268060 cm)
--(30.524670 cm, 5.299890 cm)
--(30.507300 cm, 5.326560 cm)
--(30.488520 cm, 5.354970 cm)
--(30.467910 cm, 5.376690 cm)
--(30.447300 cm, 5.398410 cm)
--(30.422820 cm, 5.420130 cm)
--(30.398340 cm, 5.441880 cm)
--(30.361920 cm, 5.464530 cm)
--(30.326850 cm, 5.481030 cm)
--(30.300150 cm, 5.482110 cm)
--(30.274380 cm, 5.479680 cm)
--(30.257040 cm, 5.458560 cm)
--(30.243840 cm, 5.429370 cm)
--(30.245790 cm, 5.390970 cm)
--(30.252900 cm, 5.371020 cm)
--(30.259920 cm, 5.347980 cm)
--(30.278700 cm, 5.314890 cm)
--(30.292050 cm, 5.297040 cm)
--(30.305220 cm, 5.275560 cm)
--(30.324600 cm, 5.250810 cm)
--(30.347610 cm, 5.220570 cm)
--(30.379380 cm, 5.183820 cm)
--(30.399960 cm, 5.163570 cm)
--(30.422820 cm, 5.141730 cm)
--(30.455970 cm, 5.118120 cm)
--(30.495600 cm, 5.097540 cm)
--(30.545760 cm, 5.084550 cm)
--(30.603030 cm, 5.084730 cm)
--(30.636540 cm, 5.094330 cm)
--(30.671070 cm, 5.106810 cm)
--(30.705270 cm, 5.129220 cm)
--(30.739500 cm, 5.155410 cm)
--(30.772890 cm, 5.193180 cm)
--(30.803370 cm, 5.237280 cm)
--(30.816630 cm, 5.263560 cm)
--(30.829860 cm, 5.289840 cm)
--(30.840960 cm, 5.318880 cm)
--(30.852030 cm, 5.347950 cm)
--(30.860460 cm, 5.383020 cm)
--(30.868890 cm, 5.418120 cm)
--(30.873450 cm, 5.455890 cm)
--(30.877980 cm, 5.493660 cm)
--(30.878430 cm, 5.534670 cm)
--(30.876750 cm, 5.576430 cm)
--(30.871950 cm, 5.619270 cm)
--(30.864960 cm, 5.662650 cm)
--(30.854130 cm, 5.708610 cm)
--(30.841110 cm, 5.754990 cm)
--(30.825300 cm, 5.802030 cm)
--(30.807420 cm, 5.849430 cm)
--(30.786300 cm, 5.898210 cm)
--(30.763530 cm, 5.947260 cm)
--(30.738150 cm, 5.997150 cm);
\fill[black,opacity=\op] (29.265000 cm, 1.860870 cm) circle (\R);
\fill[black,opacity=\op] (29.262720 cm, 2.003520 cm) circle (\R);
\fill[black,opacity=\op] (29.274390 cm, 2.135850 cm) circle (\R);
\fill[black,opacity=\op] (29.304780 cm, 2.280510 cm) circle (\R);
\fill[black,opacity=\op] (29.368590 cm, 2.418810 cm) circle (\R);
\fill[black,opacity=\op] (29.501880 cm, 2.537430 cm) circle (\R);
\fill[black,opacity=\op] (29.654070 cm, 2.559570 cm) circle (\R);
\fill[black,opacity=\op] (29.800620 cm, 2.529840 cm) circle (\R);
\fill[black,opacity=\op] (29.903490 cm, 2.490210 cm) circle (\R);
\fill[black,opacity=\op] (29.907840 cm, 2.413230 cm) circle (\R);
\fill[black,opacity=\op] (29.775750 cm, 2.363670 cm) circle (\R);
\fill[black,opacity=\op] (29.634630 cm, 2.375790 cm) circle (\R);
\fill[black,opacity=\op] (29.617710 cm, 2.418300 cm) circle (\R);
\fill[black,opacity=\op] (29.633070 cm, 2.460180 cm) circle (\R);
\fill[black,opacity=\op] (29.503380 cm, 2.472600 cm) circle (\R);
\fill[black,opacity=\op] (29.383800 cm, 2.360400 cm) circle (\R);
\fill[black,opacity=\op] (29.323440 cm, 2.188050 cm) circle (\R);
\fill[black,opacity=\op] (29.309220 cm, 1.999080 cm) circle (\R);
\fill[black,opacity=\op] (29.335980 cm, 1.995000 cm) circle (\R);
\fill[black,opacity=\op] (29.388090 cm, 2.138910 cm) circle (\R);
\fill[black,opacity=\op] (29.465760 cm, 2.251590 cm) circle (\R);
\fill[black,opacity=\op] (29.623890 cm, 2.298390 cm) circle (\R);
\fill[black,opacity=\op] (29.805420 cm, 2.305680 cm) circle (\R);
\fill[black,opacity=\op] (29.967900 cm, 2.323710 cm) circle (\R);
\fill[black,opacity=\op] (30.077250 cm, 2.366100 cm) circle (\R);
\fill[black,opacity=\op] (30.163290 cm, 2.445270 cm) circle (\R);
\fill[black,opacity=\op] (30.222360 cm, 2.509980 cm) circle (\R);
\fill[black,opacity=\op] (30.254700 cm, 2.516490 cm) circle (\R);
\fill[black,opacity=\op] (30.277770 cm, 2.466030 cm) circle (\R);
\fill[black,opacity=\op] (30.263040 cm, 2.305710 cm) circle (\R);
\fill[black,opacity=\op] (30.213240 cm, 2.186490 cm) circle (\R);
\fill[black,opacity=\op] (30.120660 cm, 2.078820 cm) circle (\R);
\fill[black,opacity=\op] (29.979720 cm, 2.015250 cm) circle (\R);
\fill[black,opacity=\op] (29.823540 cm, 2.040450 cm) circle (\R);
\fill[black,opacity=\op] (29.755320 cm, 2.121870 cm) circle (\R);
\fill[black,opacity=\op] (29.839140 cm, 2.185440 cm) circle (\R);
\fill[black,opacity=\op] (29.931360 cm, 2.161950 cm) circle (\R);
\fill[black,opacity=\op] (29.957250 cm, 2.121960 cm) circle (\R);
\fill[black,opacity=\op] (30.084630 cm, 2.201970 cm) circle (\R);
\fill[black,opacity=\op] (30.023430 cm, 2.264130 cm) circle (\R);
\fill[black,opacity=\op] (29.859120 cm, 2.269260 cm) circle (\R);
\fill[black,opacity=\op] (29.687430 cm, 2.253030 cm) circle (\R);
\fill[black,opacity=\op] (29.562210 cm, 2.189460 cm) circle (\R);
\fill[black,opacity=\op] (29.541960 cm, 2.097660 cm) circle (\R);
\fill[black,opacity=\op] (29.576040 cm, 2.039880 cm) circle (\R);
\fill[black,opacity=\op] (29.652750 cm, 1.989690 cm) circle (\R);
\fill[black,opacity=\op] (29.757990 cm, 1.955190 cm) circle (\R);
\fill[black,opacity=\op] (29.902740 cm, 1.942470 cm) circle (\R);
\fill[black,opacity=\op] (30.035820 cm, 1.970970 cm) circle (\R);
\fill[black,opacity=\op] (30.181560 cm, 2.067450 cm) circle (\R);
\fill[black,opacity=\op] (30.258060 cm, 2.168670 cm) circle (\R);
\fill[black,opacity=\op] (30.313590 cm, 2.300550 cm) circle (\R);
\fill[black,opacity=\op] (30.341700 cm, 2.458950 cm) circle (\R);
\fill[black,opacity=\op] (30.333510 cm, 2.632140 cm) circle (\R);
\fill[black,opacity=\op] (30.283260 cm, 2.810130 cm) circle (\R);
\fill[black,opacity=\op] (30.201480 cm, 2.982540 cm) circle (\R);
\fill[black,opacity=\op] (30.098730 cm, 3.151890 cm) circle (\R);
\fill[black,opacity=\op] (29.985210 cm, 3.320040 cm) circle (\R);
\fill[black,opacity=\op] (29.871300 cm, 3.493830 cm) circle (\R);
\fill[black,opacity=\op] (29.772990 cm, 3.674280 cm) circle (\R);
\fill[black,opacity=\op] (29.696070 cm, 3.854610 cm) circle (\R);
\fill[black,opacity=\op] (29.642430 cm, 4.034190 cm) circle (\R);
\fill[black,opacity=\op] (29.618760 cm, 4.206720 cm) circle (\R);
\fill[black,opacity=\op] (29.626200 cm, 4.361250 cm) circle (\R);
\fill[black,opacity=\op] (29.656740 cm, 4.486290 cm) circle (\R);
\fill[black,opacity=\op] (29.734380 cm, 4.635870 cm) circle (\R);
\fill[black,opacity=\op] (29.816070 cm, 4.723560 cm) circle (\R);
\fill[black,opacity=\op] (29.893170 cm, 4.785960 cm) circle (\R);
\fill[black,opacity=\op] (29.932800 cm, 4.848480 cm) circle (\R);
\fill[black,opacity=\op] (29.945760 cm, 4.956000 cm) circle (\R);
\fill[black,opacity=\op] (29.952600 cm, 5.077890 cm) circle (\R);
\fill[black,opacity=\op] (29.982750 cm, 5.094660 cm) circle (\R);
\fill[black,opacity=\op] (30.042480 cm, 4.942140 cm) circle (\R);
\fill[black,opacity=\op] (30.087840 cm, 4.804260 cm) circle (\R);
\fill[black,opacity=\op] (30.131460 cm, 4.644390 cm) circle (\R);
\fill[black,opacity=\op] (30.153930 cm, 4.459410 cm) circle (\R);
\fill[black,opacity=\op] (30.133110 cm, 4.293240 cm) circle (\R);
\fill[black,opacity=\op] (30.041130 cm, 4.160310 cm) circle (\R);
\fill[black,opacity=\op] (29.909670 cm, 4.217070 cm) circle (\R);
\fill[black,opacity=\op] (29.917440 cm, 4.277760 cm) circle (\R);
\fill[black,opacity=\op] (29.947050 cm, 4.323570 cm) circle (\R);
\fill[black,opacity=\op] (29.958270 cm, 4.447890 cm) circle (\R);
\fill[black,opacity=\op] (29.911830 cm, 4.536990 cm) circle (\R);
\fill[black,opacity=\op] (29.794830 cm, 4.520160 cm) circle (\R);
\fill[black,opacity=\op] (29.720100 cm, 4.409730 cm) circle (\R);
\fill[black,opacity=\op] (29.688240 cm, 4.234200 cm) circle (\R);
\fill[black,opacity=\op] (29.706090 cm, 4.070130 cm) circle (\R);
\fill[black,opacity=\op] (29.738820 cm, 3.955980 cm) circle (\R);
\fill[black,opacity=\op] (29.813430 cm, 3.788040 cm) circle (\R);
\fill[black,opacity=\op] (29.875440 cm, 3.689610 cm) circle (\R);
\fill[black,opacity=\op] (29.931000 cm, 3.662760 cm) circle (\R);
\fill[black,opacity=\op] (29.934210 cm, 3.754830 cm) circle (\R);
\fill[black,opacity=\op] (29.939940 cm, 3.878160 cm) circle (\R);
\fill[black,opacity=\op] (29.978160 cm, 3.935580 cm) circle (\R);
\fill[black,opacity=\op] (30.057450 cm, 3.997170 cm) circle (\R);
\fill[black,opacity=\op] (30.133050 cm, 4.097640 cm) circle (\R);
\fill[black,opacity=\op] (30.189030 cm, 4.249710 cm) circle (\R);
\fill[black,opacity=\op] (30.205230 cm, 4.385040 cm) circle (\R);
\fill[black,opacity=\op] (30.193590 cm, 4.560750 cm) circle (\R);
\fill[black,opacity=\op] (30.149880 cm, 4.761480 cm) circle (\R);
\fill[black,opacity=\op] (30.091380 cm, 4.972530 cm) circle (\R);
\fill[black,opacity=\op] (30.043410 cm, 5.178420 cm) circle (\R);
\fill[black,opacity=\op] (30.017430 cm, 5.366370 cm) circle (\R);
\fill[black,opacity=\op] (30.021390 cm, 5.523690 cm) circle (\R);
\fill[black,opacity=\op] (30.060630 cm, 5.664090 cm) circle (\R);
\fill[black,opacity=\op] (30.162180 cm, 5.798040 cm) circle (\R);
\fill[black,opacity=\op] (30.334260 cm, 5.825850 cm) circle (\R);
\fill[black,opacity=\op] (30.462210 cm, 5.739030 cm) circle (\R);
\fill[black,opacity=\op] (30.567810 cm, 5.603220 cm) circle (\R);
\fill[black,opacity=\op] (30.592920 cm, 5.518770 cm) circle (\R);
\fill[black,opacity=\op] (30.509250 cm, 5.496660 cm) circle (\R);
\fill[black,opacity=\op] (30.408180 cm, 5.578650 cm) circle (\R);
\fill[black,opacity=\op] (30.356430 cm, 5.668020 cm) circle (\R);
\fill[black,opacity=\op] (30.393180 cm, 5.683170 cm) circle (\R);
\fill[black,opacity=\op] (30.304020 cm, 5.775510 cm) circle (\R);
\fill[black,opacity=\op] (30.180960 cm, 5.756400 cm) circle (\R);
\fill[black,opacity=\op] (30.075000 cm, 5.598330 cm) circle (\R);
\fill[black,opacity=\op] (30.083790 cm, 5.530800 cm) circle (\R);
\fill[black,opacity=\op] (30.181200 cm, 5.622420 cm) circle (\R);
\fill[black,opacity=\op] (30.306990 cm, 5.594700 cm) circle (\R);
\fill[black,opacity=\op] (30.427560 cm, 5.490900 cm) circle (\R);
\fill[black,opacity=\op] (30.558780 cm, 5.378340 cm) circle (\R);
\fill[black,opacity=\op] (30.662520 cm, 5.343240 cm) circle (\R);
\fill[black,opacity=\op] (30.765270 cm, 5.410140 cm) circle (\R);
\fill[black,opacity=\op] (30.815070 cm, 5.478840 cm) circle (\R);
\fill[black,opacity=\op] (30.815610 cm, 5.380890 cm) circle (\R);
\fill[black,opacity=\op] (30.756540 cm, 5.248170 cm) circle (\R);
\fill[black,opacity=\op] (30.652410 cm, 5.155650 cm) circle (\R);
\fill[black,opacity=\op] (30.499440 cm, 5.173710 cm) circle (\R);
\fill[black,opacity=\op] (30.454350 cm, 5.268810 cm) circle (\R);
\fill[black,opacity=\op] (30.511140 cm, 5.256570 cm) circle (\R);
\fill[black,opacity=\op] (30.507300 cm, 5.326560 cm) circle (\R);
\fill[black,opacity=\op] (30.422820 cm, 5.420130 cm) circle (\R);
\fill[black,opacity=\op] (30.300150 cm, 5.482110 cm) circle (\R);
\fill[black,opacity=\op] (30.245790 cm, 5.390970 cm) circle (\R);
\fill[black,opacity=\op] (30.292050 cm, 5.297040 cm) circle (\R);
\fill[black,opacity=\op] (30.379380 cm, 5.183820 cm) circle (\R);
\fill[black,opacity=\op] (30.495600 cm, 5.097540 cm) circle (\R);
\fill[black,opacity=\op] (30.671070 cm, 5.106810 cm) circle (\R);
\fill[black,opacity=\op] (30.803370 cm, 5.237280 cm) circle (\R);
\fill[black,opacity=\op] (30.852030 cm, 5.347950 cm) circle (\R);
\fill[black,opacity=\op] (30.877980 cm, 5.493660 cm) circle (\R);
\fill[black,opacity=\op] (30.864960 cm, 5.662650 cm) circle (\R);
\fill[black,opacity=\op] (30.807420 cm, 5.849430 cm) circle (\R);
